Open Visual Knowledge Extraction via Relation-Oriented Multimodality Model Prompting

Images contain rich relational knowledge that can help machines understand the world. Existing methods on visual knowledge extraction often rely on the pre-defined format (e.g., sub-verb-obj tuples) or vocabulary (e.g., relation types), restricting the expressiveness of the extracted knowledge. In this work, we take a first exploration to a new paradigm of open visual knowledge extraction. To achieve this, we present OpenVik which consists of an open relational region detector to detect regions potentially containing relational knowledge and a visual knowledge generator that generates format-free knowledge by prompting the large multimodality model with the detected region of interest. We also explore two data enhancement techniques for diversifying the generated format-free visual knowledge. Extensive knowledge quality evaluations highlight the correctness and uniqueness of the extracted open visual knowledge by OpenVik. Moreover, integrating our extracted knowledge across various visual reasoning applications shows consistent improvements, indicating the real-world applicability of OpenVik.

==> sections/09-rebuttal.tex <==
% notation meaning summary
\begin{minipage}{\textwidth}
\begin{minipage}[t]{0.49\textwidth}
\makeatletter\def\@captype{table}
\captionof{table}{Notations for region detector.}
\label{tab:hype4detector}
\resizebox{\linewidth}{!}{%
\begin{tabular}{c|c}
\toprule
\textbf{Notation} & \textbf{Meaning} \\
\midrule
$\mathcal{L}_\text{RD}$ & region regression loss supervised by union regional boxes\\
$\mathcal{L}_\text{K}$ & knowledge generation loss supervised by GT relational knowledge  \\
$\mathcal{L}_v$ & the overall objective of the relational region detector \\
$\mathcal{I}_i$ & input image of the relational region detector\\
$\mathcal{U}_j$ & relation-centric box label \\
$\mathbf{U}_i$ & set of relation-centric boxes of an image \\ 
$\mathcal{T}_j$ & region description of a box\\
$\mathbf{T}_i$ & set of region descriptions of the an image \\ 
\bottomrule
\end{tabular}
}
\end{minipage}
\qquad
\begin{minipage}[t]{0.49\textwidth}
\makeatletter\def\@captype{table}
\captionof{table}{Notations for knowledge generator.}
\label{tab:hype4generator}
\resizebox{\linewidth}{!}{%
\begin{tabular}{c|c}
\toprule
\textbf{Notation} & \textbf{Meaning} \\
\midrule
$\mathcal{L}_{\text{V}}$ & inter-sequence language diversity regularizer \\
$\mathcal{L}_l$ & the overall objective of the knowledge generator \\
$\mathcal{I}_i$ & the input image of the knowledge generator\\
$N_i$ & the number of generated knowledge descriptions of an image \\
$T_a, T_b$ & two regional knowledge descriptions of one same image \\
$s (T_a, T_b)$ & the semantic cosine similarity of two input generated descriptions \\
$\phi$ & hyper-parameter controlling the penalty slightly different sequences \\
$\alpha$ & weight hyper-parameter balancing generation accuracy and diversity \\
\bottomrule
\end{tabular}
}
\end{minipage}
\end{minipage}

% enriched baselines (also contained in markdown)
\begin{table*}[h]
\centering
% \small
% \vskip -1.1em
\caption{Enriched baselines for knowledge generation on performance and in-depth quality (\%). }
\label{tab:performance}
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{l|ccc|cccc}
\toprule
\multirow{2.5}{*}{\bf Method} &\multicolumn{3}{c|}{{\cellcolor{maroon}}{\bf Generation Performance}} &  \multicolumn{4}{c}{\cellcolor{lightblue}{\bf In-Depth Knowledge Quality}}\\
\cmidrule(lr){2-4} \cmidrule(lr){5-8} 
& {BLEU$\uparrow$} & {ROUGE-L$\uparrow$} & {METEOR$\uparrow$} &  {Validity$\uparrow$} & {Conformity$\uparrow$} & {Freshness$\uparrow$} & {Diversity$\uparrow$} \\
% \hline 
% \midrule
% \multirow{3}{*}{\thead{Training Data}}
% \rowcolor{gray!15}\multicolumn{8}{l}{\emph{Training Data}}  \\
% \hline 
% \midrule
% Visual Genome~\cite{krishna2017visual} & --- & --- & --- &  --- & --- & --- & 0.675  \\
% Relational Caps~\cite{kim2019dense} & --- & --- & --- &  --- & --- & --- & 0.684 \\
% Diversity Enhanced & --- & --- &  --- &  --- & --- & --- &  \\
% \hline 
% \midrule
% \multirow{4}{*}{\thead{Scene Graph \\ Generation}}
% \rowcolor{gray!15}\multicolumn{8}{l}{\emph{Closed/Open Scene Graph Generation}}  \\
% % \hline 
% IMP~\cite{xu2017scene} & 0.075 & 0.123 & 0.118 &  0.800 & 0.823 & 0.676 & 0.316 \\
% Neural Motifs~\cite{zellers2018neural} & 0.229 & \underline{0.283} & \underline{0.273}  & 0.822 & 0.767 & 0.667 & 0.349 \\
% UnbiasSGG~\cite{tang2020unbiased} & 0.217 & 0.258 & 0.194 & 0.739 & 0.733 & 0.666 & 0.357\\
% Ov-SGG~\cite{he2022towards} & 0.167 & 0.210 & 0.183 & 0.712 & 0.633 & 0.693 & 0.413 \\
% \hline 
\midrule
% & GB-NET &  &  &  &  &  &  &  &  \\
% \multirow{2}{*}{\thead{Open Vocabulary SGG}}
% & Ov-SGG &  &  &  &  &  &  &  &  \\
% & CaCao &  &  &  &  &  &  &  &  \\
% \midrule
% \multirow{1}{*}{Dense Captioning} 
\rowcolor{gray!15}\multicolumn{8}{l}{\emph{Region Captioning}}  \\
% \hline 
DenseCap~\cite{densecap} & 0.248 & 0.245 & 0.196  & 0.883 & 0.843 & 0.790 & 0.543 \\
Sub-GC~\cite{zhong2020comprehensive} & 0.272 & 0.263 & 0.221  & 0.892 & \underline{0.871} & \underline{0.795} & \underline{0.547} \\
BLIP~\cite{DBLP:conf/icml/0001LXH22} & 0.264 & 0.266 & \underline{0.252}  & 0.886 & 0.855 & 0.760 & 0.531 \\
BLIP2~\cite{li2023blip} & \underline{0.275} & \textbf{0.285} & \textbf{0.257}  & 0.892 & \underline{0.871} & 0.766 & 0.535 \\
% GRiT~\cite{wu2022grit} & \bf 0.333 & \bf 0.313 & \bf 0.292  & 0.895 & \underline{0.879} & \underline{0.803} & \underline{0.585} \\
% \hline
% \midrule
% \multirow{1}{*}{Relational Captioning} 
% \rowcolor{gray!15}\multicolumn{8}{l}{\emph{Dense Relational Captioning}}  \\
% \hline 
% & TSNet & 0.61 & 32.36 & 16.09 &  &  &  &  &  \\
% & MTTSNet & 0.88  & 34.27  & 18.73  &  &  &  &  &  &  \\
% & \multirow{2}{*}{MTTSNet+REM} & \multirow{2}{*}{1.12}  & \multirow{2}{*}{45.96}  & \multirow{2}{*}{0.184}  & \multirow{2}{*}{} & \multirow{2}{*}{} &  & \multirow{2}{*}{} & \multirow{2}{*}{} & \multirow{2}{*}{} \\ \\
MTTSNet+REM~\cite{kim2019dense} & 0.240 & 0.226 & 0.228  & \underline{0.897} & 0.852 &  0.754 & 0.375 \\
% \hline 
\midrule
% \multirow{1}{*}{Ours} 
\rowcolor{gray!15}\multicolumn{8}{l}{\emph{Ours}}  \\
% \hline 
% \midrule 
\ours & \textbf{0.280} & \underline{0.283} & \underline{0.250} &  \bf 0.907 & \bf 0.883 & \bf 0.809 & \bf 0.619 \\
% 0.643
\bottomrule
\end{tabular}
}
% \vskip -0.5em
\end{table*}

% \begin{wrapfigure}{r}{1\textwidth}
% \includegraphics[width=0.8\linewidth]{figures/ablation-new.pdf} 
% % \vskip -0.5em
% \centering
% \caption{The influence of knowledge diversity regularization and diversity-driven data enhancement strategies.}
% % \vskip -1.0em
% \label{fig:ablation}
% \end{wrapfigure}

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/ablation-new.pdf}
    % \vskip -1.0em
    \caption{Add ablation results on the pre-trained detector.}
    \label{fig:ablation_new}
\end{figure}

% additional backbone for three applications (also contained in markdown)
\begin{figure}[ht]
\begin{minipage}[c]{0.33\linewidth}
% \vskip -1.4em
\centering
\captionof{table}{Application: Retrieval}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|ccccc}
\toprule
\textbf{Method} & \textbf{Recall@1} & \textbf{Recall@5}  & \textbf{Recall@10} & \textbf{\textit{Avg}}   \\
\midrule
% Zero-Shot & 0.36156351791530944 & 0.6547231270358306 & 0.7866449511400652 & 0.6009771986970684 &  \\
% \ours Context+ & 0.40553745928338764 & 0.7328990228013029 & 0.8452768729641694 & 0.6612377850162866 & \\
ZS-CLIP & 36.16 & 65.47 & 78.66 & 60.10 &  \\
\rowcolor{gray!15}\ours + ZS-CLIP & 40.55 & 73.29 & 84.53 & 66.12 & \\
BLIP & 63.11 & 86.30 & 91.10 & 80.17 &  \\
\rowcolor{gray!15}\ours + BLIP & 65.23 & 87.71 & 91.90 & 81.61 & \\
\bottomrule
\end{tabular}
}
\label{tab:ir}
\end{minipage}
\hfill
\begin{minipage}[c]{0.31\linewidth}
\centering
\captionof{table}{Application: GSR.}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|ccccc}
\toprule
\textbf{Method} & \textbf{Accuracy} & \textbf{Precision}  & \textbf{Recall} & \textbf{$\text{F}_1$}   \\
\midrule
ZS-CLIP & 53.14 & 42.54 & 45.19 & 41.78 &  \\
\rowcolor{gray!15}\ours + ZS-CLIP & 75.16 & 61.63 & 62.75 & 61.03 &  \\
BLIP & 70.42 & 65.32 & 69.25 & 67.23 &  \\
\rowcolor{gray!15}\ours + BLIP & 80.25 & 72.55 & 70.61 & 71.57 & \\
\bottomrule
\end{tabular}
}
\label{tab:gsr}
\end{minipage}
\hfill
\begin{minipage}[c]{0.31\linewidth}
\centering
\captionof{table}{Application: VCR.}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|ccccc}
\toprule
\textbf{Method} & \textbf{Accuracy} & \textbf{Precision}  & \textbf{Recall} & \textbf{$\text{F}_1$}   \\
\midrule
ZS-CLIP  & 56.66 & 56.73 & 56.72 & 56.66 &  \\
\rowcolor{gray!15}\ours + ZS-CLIP & 59.96 & 60.01 & 60.03 & 59.95 &  \\
R2C & 62.50 & 62.50 & 62.45 & 62.47 &  \\
\rowcolor{gray!15}\ours + R2C & 67.40 & 67.54 & 67.43 & 67.48 &  \\
\bottomrule
\end{tabular}
}
\label{tab:vcr}
\end{minipage}
\end{figure}


\begin{figure}[h!]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/failure_case.pdf}
    \caption{Examples of incorrectly inferred knowledge resulting from distribution bias are {\colorbox{case_error}{highlighted}}.}
    \label{fig:failure_case}
\end{figure}

==> tables/main_exp.tex <==
\begin{table*}[h]
\centering
\small
\caption{Generation performance comparison and in-depth knowledge quality comparison with different baselines and the original training data (\%). }
\label{tab:main_exp}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{cccccccccc}
\toprule
\multirow{2.5}{*}{Type} & \multirow{2.5}{*}{Data/Method} &\multicolumn{3}{c}{\bf Generation Performance} & & \multicolumn{4}{c}{\bf In-Depth Knowledge Quality}\\
\cmidrule(lr){3-5} \cmidrule(lr){7-10} 
& & \textit{BLEU-1$\uparrow$} & \textit{ROUGE-L$\uparrow$} & \textit{METEOR$\uparrow$} &  & \textit{Validity$\uparrow$} & \textit{Conformity$\uparrow$} & \textit{Freshness$\uparrow$} & \textit{Diversity$\uparrow$} \\
\midrule
\multirow{3}{*}{\thead{Training Data}}
& Visual Genome & --- & --- & --- &  & --- & --- & --- & 0.675  \\
& Relational Caps & --- & --- & --- &  & --- & --- & --- & 0.684 \\
& \cellcolor{gray!20} Diversity Enhanced & \cellcolor{gray!20} --- & \cellcolor{gray!20} --- & \cellcolor{gray!20} --- & \cellcolor{gray!20} & \cellcolor{gray!20} --- & \cellcolor{gray!20} --- & \cellcolor{gray!20} --- & \cellcolor{gray!20} \\
\midrule
\multirow{4}{*}{\thead{Scene Graph \\ Generation}}
& IMP & 0.135 & 0.123 & 0.118 &  & 0.8 & 0.843 &  & 0.485 \\
& Neural Motifs & 0.329 & 0.283 & 0.273 &  & 0.822 & 0.767 &  & 0.556 \\
& UnbiasSGG & 0.305 & 0.258 & 0.194 &  & 0.867 & 0.733 &  & 0.534\\
& Ov-SGG &  &  &  &  &  &  &  &  \\
% & GB-NET &  &  &  &  &  &  &  &  \\
\midrule
% \multirow{2}{*}{\thead{Open Vocabulary SGG}}
% & Ov-SGG &  &  &  &  &  &  &  &  \\
% & CaCao &  &  &  &  &  &  &  &  \\
% \midrule
\multirow{1}{*}{Dense Captioning} 
& DenseCap &  &  & 0.196 &  &  &  &  \\
\midrule
\multirow{1}{*}{Relational Captioning} 
% & TSNet & 0.61 & 32.36 & 16.09 &  &  &  &  &  \\
% & MTTSNet & 0.88  & 34.27  & 18.73  &  &  &  &  &  &  \\
% & \multirow{2}{*}{MTTSNet+REM} & \multirow{2}{*}{1.12}  & \multirow{2}{*}{45.96}  & \multirow{2}{*}{0.184}  & \multirow{2}{*}{} & \multirow{2}{*}{} &  & \multirow{2}{*}{} & \multirow{2}{*}{} & \multirow{2}{*}{} \\ \\
& MTTSNet+REM & 0.295 & 0.234 & 0.220  &  &  &  &  & 0.286 \\ 
\midrule
\multirow{1}{*}{Ours} 
& \cellcolor{gray!20} \ours & \cellcolor{gray!20} 0.388 & \cellcolor{gray!20} 0.283 & \cellcolor{gray!20} 0.250 & \cellcolor{gray!20} & \cellcolor{gray!20} 0.967 & \cellcolor{gray!20} 0.933 & \cellcolor{gray!20} & \cellcolor{gray!20} \\
% 0.643
\bottomrule
\end{tabular}
}
\end{table*}
